VSFormer: Value and Shape-Aware Transformer with Prior-Enhanced Self-Attention for Multivariate Time Series Classification

Multivariate time series classification is a crucial task in data mining, attracting growing research interest due to its broad applications. While many existing methods focus on discovering discriminative patterns in time series, real-world data does not always present such patterns, and sometimes raw numerical values can also serve as discriminative features. Additionally, the recent success of Transformer models has inspired many studies. However, when applying to time series classification, the self-attention mechanisms in Transformer models could introduce classification-irrelevant features, thereby compromising accuracy. To address these challenges, we propose a novel method, VSFormer, that incorporates both discriminative patterns (shape) and numerical information (value). In addition, we extract class-specific prior information derived from supervised information to enrich the positional encoding and provide classification-oriented self-attention learning, thereby enhancing its effectiveness. Extensive experiments on all 30 UEA archived datasets demonstrate the superior performance of our method compared to SOTA models. Through ablation studies, we demonstrate the effectiveness of the improved encoding layer and the proposed self-attention mechanism. Finally, We provide a case study on a real-world time series dataset without discriminative patterns to interpret our model.

==> Notation.tex <==
\section{Problem Formulation}
A multivariate time series (MTS), $\mathbf{X} = \{X^1,...,X^V\} \in \mathbb{R}^{V \times T}$, is a collection of several univariate time series, $X^i \in \{x_1,...,x_T\}$. Here, $T\in \mathbb{Z}^+$ is the total number of observations, and $V\in\mathbb{Z}^+$ represents the number of variables.

An MTS dataset consists of pairs of MTS and associated labels, which can be represented as $\{(\mathbf{X}_1, y_1),...,(\mathbf{X}_N, y_N)\}$. Here, $y = \{y_1,...,y_C\}\in\mathbb{R}^C$ denotes the corresponding class, and $N$ is the total count of MTS instances in the dataset.

A multivariate time series classification (MTSC) problem aims to train a classifier that can predict the class label for an unlabeled, previously unseen MTS.
